Evaluating Geospatial RDF stores Using the Benchmark Geographica 2

Since 2007, geospatial extensions of SPARQL, like GeoSPARQL and stSPARQL, have been defined and corresponding geospatial RDF stores have been implemented. In addition, some work on developing benchmarks for evaluating geospatial RDF stores has been carried out. In this paper, we revisit the Geographica benchmark defined by our group in 2013 which uses both real world and synthetic data to test the performance and functionality of geospatial RDF stores. We present Geographica 2, a new version of the benchmark which extends Geographica by adding one more workload, extending our existing workloads and evaluating 5 more RDF stores. Using three different real workloads, Geographica 2 tests the efficiency of primitive spatial functions in RDF stores and the performance of the RDF stores in real use case scenarios, a more detailed evaluation is performed using a synthetic workload and the scalability of the RDF stores is stressed with the scalability workload. In total eight systems are evaluated out of which six adequately support GeoSPARQL and two offer limited spatial support.

==> common-preamble.tex <==

%Greek
%\usepackage[greek,english]{babel}
%\usepackage[utf8x]{inputenc}
%\newcommand{\gr}{\selectlanguage{greek}}
%\newcommand{\en}{\selectlanguage{english}}
\usepackage[greek,english]{babel} 
%
\usepackage{makeidx}  % allows for indexgeneration
%
\usepackage{ulem}
\usepackage{longtable}
\usepackage{amssymb}
\usepackage{multirow}
\usepackage{enumitem}

\usepackage{lscape}
\usepackage{subfigure}
\usepackage{caption}
\usepackage{graphicx}

\usepackage{float}
\usepackage[disable]{todonotes}
%\usepackage{todonotes}
\restylefloat{table}

\usepackage{textcomp}

\usepackage{color}
\usepackage{soul}
\usepackage{verbatim}

\usepackage[font=small,labelfont=bf]{caption}

\usepackage{afterpage}
\usepackage{comment}
%\usepackage{subfig}
%\usepackage{booktabs}

\definecolor{darkgreen}{rgb}{0,0.392,0}
\definecolor{darkred}{rgb}{0.545,0,0}

\newcommand{\sppbench}{\(\mathrm{SP^{2}Bench}\)}
\newcommand{\dg}{\color{darkgreen}}
\newcommand{\dr}{\color{darkred}}
\newcommand{\cm}[1]{\includecomment{#1}}
\newcommand{\colbreak}{\hspace{20pt}}	% Adds a horizontal space equal 
										% to space between document columnts

\usepackage{siunitx}
\sisetup{input-symbols = {()},  % do not treat "(" and ")" in any special way
         group-digits  = false} % no grouping of digits
         

% #006400 green
% #910D0D red
\definecolor{my-green}{rgb}{0,0.39,0}
\definecolor{my-red}{rgb}{0.57,0.05,0.05}
\newcommand{\green}[1]{\textcolor{my-green}{#1}}
\newcommand{\red}[1]{\textcolor{red}{#1}}

\newcommand{\ftodo}{\todo[fancyline]}
\newcommand{\todoA}{\todo[color=green]}
\newcommand{\todoB}{\todo[color=yellow]}
\newcommand{\todoC}{\todo[color=red]}


==> functional-table.tex <==
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
{\scriptsize
\begin{table*}[t]
% \begin{table}[htbp]
\centering
\scriptsize
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
System						& Strabon	& uSeekM	& Parliament	& System X	& Virtuoso 	& System Y	& OWLIM \\
\end{tabular}}
\caption{Functionality of geospatial RDF stores}
\label{tab:functional-comparison}
\end{table*}
}


==> resultsRealMicroTable.tex <==

\begin{table*}[!t]
\tiny
\centering
%\begin{tabular}{|l|l|c|c|c|c|c|c|}
\resizebox{\textwidth}{!}{
%\begin{tabular}{|m{40pt}|l|S|S|S|c|c|S||S|S|S|c|c|S|} %[table-format=4.2]}
\begin{tabular}{|m{40pt}|l|c|c|c|c|c|c|c||c|c|c|c|c|c|c|}
\hline
\multirow{3}{*}{\textbf{Type}} & \multirow{3}{*}{\textbf{Query}} & \multicolumn{7}{c||}{\textbf{Cold caches} (sec.)} & \multicolumn{7}{c|}{\textbf{Warm caches} (sec.)} \\
\cline{3-16}    
&	& \multirow{2}{*}{\textbf{Strabon}}	& \multirow{2}{*}{\textbf{uSeekM}} & \multirow{2}{*}{\textbf{Parliament}} & \multicolumn{2}{c|}{\textbf{System X}}	& \multirow{2}{*}{\textbf{GraphDB}}	& \multirow{2}{*}{\textbf{RDF4J}} & \multirow{2}{*}{\textbf{Strabon}}	& \multirow{2}{*}{\textbf{uSeekM}}	&	\multirow{2}{*}{\textbf{Parliament}}	& \multicolumn{2}{c|}{\textbf{System X}}  & \multirow{2}{*}{\textbf{GraphDB}}  & \multirow{2}{*}{\textbf{RDF4J}} \\
\cline{6-7} \cline{13-14} 
&	& & & & Parallel & Serial & & \textit{(Lucene enabled)} & &	& & Parallel & Serial & & \textit{(Lucene enabled)} \\
\hline \hline                                   		                                		                                			                                                                                                    		                                		                                				                                	            		                                
\multirow{6}{40pt}{\textbf{Non topological construct functions}}                		                                			                                                                                                    		                                		                                				                                	            		                                
& \textbf{Q1} & 42.33 & 38.11 & 152.71 & 62.58 & \color{darkred}293.85 & \color{darkgreen}29.68	& 37.34 & 41.36	& 36.25	& 132.67 & 57.45 & \color{darkred}296.96 & \color{darkgreen}27.36 & 37.20	\\ \cline{2-16}
& \textbf{Q2} & 22.48 & 21.47 & 90.23 & 44.02 & \color{darkred}204.65 & \color{darkgreen}14.55 & 18,75 & 21.06 & 19.35	& 70.62	& 35.35 & \color{darkred}187.71 & \color{darkgreen}13.26 & 17.96 \\ \cline{2-16}
& \textbf{Q3} & 29.48 & 27.06 & 98.56 & 45.86 & \color{darkred}213.47 & \color{darkgreen}19.42 & 24.56 & 27.73 & 24.13 & 79.40 & 38.25 & \color{darkred}206.70 & \color{darkgreen}18.17 & 24.11 \\ \cline{2-16}
& \textbf{Q4} & 7.65 & 3.22 & 23.16 & 19.62 & \color{darkred}309.00 & \color{darkgreen}3.20 & 3.48 & 7.00 & 3.08 & 19.67 & 19.76 & \color{darkred}334.93 & \color{darkgreen}2.15 & 3.12 \\ \cline{2-16}
& \textbf{Q5} & 14.68 & \color{darkgreen}4.17 & 21.63 & 23.60 & \color{darkred}236.60 & 7.45 & 4.64 & 13.78 & 5.00 & 19.58 & 17.41 & \color{darkred}233.53 & 6.66 & \color{darkgreen}4.47 \\ \cline{2-16}
& \textbf{Q6} & 23.82 & 19.58 & \mbox{-} & 39.87 & \color{darkred}199.25 & \color{darkgreen}13.53 & \mbox{-} & 21.06 & 18.35 & \mbox{-} & 31.58 & \color{darkred}160.40 & \color{darkgreen}12.67 & \mbox{-}\\ \cline{2-16}
\hline \hline                                   		                                		                                			                                                                                                    		                                		                                				                                                	                                                   
\multirow{11}{40pt}{\textbf{Spatial selections}} 
& \textbf{Q7} & \color{darkgreen}0.36 & 1.22 & 2.42 & long string & long string & \color{darkred}5.33 & 3.97 & \color{darkgreen}0.01 & 0.02 & 1.36 & long string & long string & \color{darkred}4.66 & 3.46 \\ \cline{2-16}
& \textbf{Q8} & \color{darkgreen}0.42 & 0.57 & \color{darkred}7.69 & long string & long string & 2.04 & 1.78 & 0.06 & \color{darkgreen}0.05 & \color{darkred}5.84 & long string & long string & 1.64 & 1.55 \\ \cline{2-16}
& \textbf{Q9} & \color{darkgreen}0.83 & 1.27 & 35.03 & long string & long string & 28.28 & \color{darkred}40.60 & 0.16 & \color{darkgreen}0.05 & 34.09 & long string & long string & 27.95 & \color{darkred}40.77 \\ \cline{2-16}
& \textbf{Q10} & \color{darkgreen}0.73 & 1.51 & \color{darkred}76.85 & long string & long string & 22.24 & 25.24 & 0.13 & \color{darkgreen}0.10 & \color{darkred}57.18 & long string & long string & 21.24 & 24.14 \\ \cline{2-16}
& \textbf{Q11} & \color{darkgreen}2.66 & 2.96 & \color{darkred}195.87 & long string & long string & 114.29 & 164.84 & 2.03 & \color{darkgreen}1.29 & \color{darkred}175.98 & long string & long string & 114.95 & 163.44 \\ \cline{2-16}
& \textbf{Q12} & 0.79 & \color{darkgreen}0.55 & 2.39 & \color{darkred}8.87 & 6.07 & 1.02 & 0.67 & 0.38 & \color{darkgreen}0.03 & 1.20 & \color{darkred}4.02 & 3.99 & 0.67 & 0.57 \\ \cline{2-16}
& \textbf{Q13} & \color{darkgreen}0.82 & 0.89 & 63.14 & long string & long string & 49.67 & \color{darkred}72.20 & 0.13 & \color{darkgreen}0.04 & 59.60 & long string & long string & 49.65 & \color{darkred}71.92 \\ \cline{2-16}
& \textbf{Q14} & \color{darkgreen}0.50 & 2.29 & \color{darkred}24.34 & 13.33 & 11.35 & 4.13 & 1.90 & \color{darkgreen}0.03 & 1.63 & \color{darkred}19.97 & 4.12 & 4.03 & 3.11 & 1.68 \\ \cline{2-16}
& \textbf{Q15} & 0.50 & 0.99 & 3.44 & 10.24 & \color{darkred}10.27 & 0.93 & \color{darkgreen}0.48 & \color{darkgreen}0.12 & 0.30 & 0.56 & 3.94 & \color{darkred}3.97 & 0.30 & 0.26 \\ \cline{2-16}
& \textbf{Q16} & \color{darkgreen}2.79 & 5.52 & 63.20 & long string & long string & 50.61 & \color{darkred}72.34 & 2.19 & \color{darkgreen}1.96 & 59.85 & long string & long string & 49.68 & \color{darkred}71.97 \\ \cline{2-16}
& \textbf{Q17} & 3.06 & \color{darkgreen}1.60 & 35.89 & long string & long string & 28.31 & \color{darkred}40.06 & 2.62 & \color{darkgreen}0.86 & 34.39 & long string & long string & 27.66 & \color{darkred}39.93 \\ \cline{2-16}
\hline \hline                                   		                                		                                			                                                                                                    		                                		                                				                                	                    		                                               
\multirow{10}{40pt}{\textbf{Spatial joins}}     		                                		                                			                                                                                                    		                                		                                				                                	                    		                                               
& \textbf{Q18} & \color{darkgreen}4.52 & 2233.73 & 2880.20 & \color{darkred}\mbox{>1h} & 14.51 & 942.89 & 2885.72 & \color{darkgreen}3.98 & 2504.24 & 2875.02 & \color{darkred}\mbox{>1h} & 11.53 & 903.33 & 2969.07 \\ \cline{2-16}
& \textbf{Q19} & \color{darkgreen}1272.54 & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} & \color{darkgreen}1284.62 & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} \\ \cline{2-16}
& \textbf{Q20} & \color{darkgreen}115.93 & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} & 396.29 & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} & \color{darkgreen}105.39 & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} & 365.01 & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} \\ \cline{2-16}
& \textbf{Q21} & \color{darkgreen}113.26 & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} & 409.54 & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} & \color{darkgreen}107.76 & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} & 364.32 & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} \\ \cline{2-16}
& \textbf{Q22} & \color{darkgreen}26.33 & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} & internal error & internal error & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} & \color{darkgreen}25.20 & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} & internal error & internal error & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} \\ \cline{2-16}
& \textbf{Q23} & \color{darkgreen}26.29 & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} & internal error & internal error & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} & \color{darkgreen}25.01 & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} & internal error & internal error & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} \\ \cline{2-16}
& \textbf{Q24} & \color{darkgreen}26.66 & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} & internal error & internal error & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} & \color{darkgreen}25.37 & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} & internal error & internal error & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} \\ \cline{2-16}
& \textbf{Q25} & \color{darkgreen}342.87 & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} & 1,629.45 & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} & \color{darkgreen}341.04 & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} & 1,577.89 & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} \\ \cline{2-16}
& \textbf{Q26} & 343.30 & 534.61 & 2040.00 & 909.18 & \color{darkred}\mbox{>1h} & 466.86 & \color{darkgreen}324.79 & 341.28 & 534.15 & 2030.42 & 955.21 & \color{darkred}\mbox{>1h} & 465.35 & \color{darkgreen}324.04 \\ \cline{2-16}
& \textbf{Q27} & \color{darkgreen}343.72 & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} & internal error & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} & \color{darkgreen}342.06 & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} & internal error & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} & \color{darkred}\mbox{>1h} \\ \cline{2-16}
\hline \hline                                   		                                		                                			                                                                                                    		                                		                                				                                              	                                            
\multirow{2}{40pt}{\textbf{Aggregate functions}}		                                		                                			                                                                                                    		                                		                                				                                              	                                                    
& \textbf{Q28} & \color{darkgreen}3.56 & \mbox{-} & \mbox{-} & \mbox{-} &  \mbox{-} & \mbox{-} & \mbox{-} & \color{darkgreen}2.92 & \mbox{-} & \mbox{-} & \mbox{-} & \mbox{-} & \mbox{-} & \mbox{-} \\ \cline{2-16}
& \textbf{Q29} & \color{darkgreen}258.35 & \mbox{-} & \mbox{-} & \mbox{-} & \mbox{-} & \mbox{-} & \mbox{-} & \color{darkgreen}258.00 & \mbox{-} & \mbox{-} & \mbox{-} & \mbox{-} & \mbox{-} & \mbox{-} \\ \cline{2-16}
\hline
\end{tabular}}
\caption{Response times - real-world workload}
\label{table:RealResponseTimes}
\end{table*}


==> syntheticResultsTable.tex <==
\iflong
\else
	\begin{landscape}
	\begin{figure*}[f]
	  \centering
		\vspace{-6em}
		  \subfigure[][\shortstack{Intersects\\ \small{ tag 1, cold caches}}]
		  {\includegraphics{graphs/synthetic/synthetic-selections-Intersects-1-cold.pdf}
		  \label{fig:SyntheticIntersects1Cold}}
		  \hspace{-1em}
		  \subfigure[][\shortstack{Intersects\\ \small{ tag 512, cold caches}}]
		  {\includegraphics{graphs/synthetic/synthetic-selections-Intersects-512-cold.pdf}
		  \label{fig:SyntheticIntersects512Cold}}
		  \hspace{-1em}
		  \subfigure[][\shortstack{Within\\ \small{ tag 1, cold caches}}]
		  {\includegraphics{graphs/synthetic/synthetic-selections-Within-1-cold.pdf}
		  \label{fig:SyntheticWithin1Cold}}
		  \hspace{-1em}
		  \subfigure[][\shortstack{Within\\ \small{tag 512, cold caches}}]
		  {\includegraphics{graphs/synthetic/synthetic-selections-Within-512-cold.pdf}
		  \label{fig:SyntheticWithin512Cold}}
		  \hspace{-1em}
		  \\
		  \subfigure[][\shortstack{Intersects\\ \small{ tag 1, warm caches}}]
		  {\includegraphics{graphs/synthetic/synthetic-selections-Intersects-1-warm.pdf}
		  \label{fig:SyntheticIntersects1Warm}}
		  \hspace{-1em}
		  \subfigure[][\shortstack{Intersects\\ \small{ tag 512, warm caches}}]
		  {\includegraphics{graphs/synthetic/synthetic-selections-Intersects-512-warm.pdf}
		  \label{fig:SyntheticIntersects512Warm}}
		  \hspace{-1em}
		  \subfigure[][\shortstack{Within\\ \small{ tag 1, warm caches}}]
		  {\includegraphics{graphs/synthetic/synthetic-selections-Within-1-warm.pdf}
		  \label{fig:SyntheticWithin1Warm}}
		  \hspace{-1em}
		  \subfigure[][\shortstack{Within\\ \small{ tag 512, warm caches}}]
		  {\includegraphics{graphs/synthetic/synthetic-selections-Within-512-warm.pdf}
		  \label{fig:SyntheticWithin512Warm}}
		  \hspace{-1em}
		  \\
	%	  \subfigure[][Spatial Joins]
	%	  {\includegraphics{graphs/synthetic/synthetic-joins.pdf}
	%	  \label{fig:SyntheticJoin}}
	%	  \hspace{-1em}
	%	  \\
		  \subfigure[][Intersects]
		  {\includegraphics[scale=0.62]{graphs/synthetic/synthetic-joins-Intersects.pdf}
		  \label{fig:SyntheticJoinIntersects}}	
		  \subfigure[][Touches]
		  {\includegraphics[scale=0.62]{graphs/synthetic/synthetic-joins-Touches.pdf}
		  \label{fig:SyntheticJoinTouches}}
		  \subfigure[][Within]
		  {\includegraphics[scale=0.62]{graphs/synthetic/synthetic-joins-Within.pdf}
		  \label{fig:SyntheticJoinWithin}}
		  \\
		\caption{Response times  - Synthetic Workload}
		\label{fig:SyntheticResponseTimes}
	\end{figure*}
	\end{landscape}
\fi


==> tabular_tex/results_macro.tex <==
\begin{table*}[!t]
	\tiny
	\centering
	\resizebox{\textwidth}{!}{
		\begin{tabular}{|m{40pt}|c|c|c|c|c|c|} %[table-format=4.2]}
			\hline
			\multirow{2}{*}{\textbf{Scenario}} & \multirow{2}{*}{\textbf{Strabon}} & \multirow{2}{*}{\textbf{uSeekM}} & \multirow{2}{*}{\textbf{Parliament}} & \multicolumn{2}{c|}{\textbf{SystemX}} & \multirow{2}{*}{\textbf{GraphDB}} \\
			\cline{5-6} & & & &	Par. & Ser. & \\
			\hline
			Reverse	Geocoding & \color{darkred}65->4.30 & 0.77 & 2.6 & 15.07 & 15.16 & \color{darkgreen}0.62 \\ 
			\hline
			Map Search and Browsing & \color{darkgreen}0.2 & 0.6 & 22.2 & 22.14 & \color{darkred}124.49 & 1.14 \\ 
			\hline
			Rapid Mapping for Fire Monitoring & \color{darkgreen}102.82 & - & - & - & - & - \\ 
			\hline
		\end{tabular}}
		\captionof{table}{Average Iteration Times - Macro Scenarios}		
		\label{table:MacroResults}
\end{table*}

